Adapting Dual-encoder Vision-language Models for Paraphrased Retrieval

In the recent years, the dual-encoder vision-language models (\eg CLIP) have achieved remarkable text-to-image retrieval performance. However, we discover that these models usually results in very different retrievals for a pair of paraphrased queries. Such behavior might render the retrieval system less predictable and lead to user frustration. In this work, we consider the task of paraphrased text-to-image retrieval where a model aims to return similar results given a pair of paraphrased queries. To start with, we collect a dataset of paraphrased image descriptions to facilitate quantitative evaluation for this task. We then hypothesize that the undesired behavior of existing dual-encoder model is due to their text towers which are trained on image-sentence pairs and lack the ability to capture the semantic similarity between paraphrased queries. To improve on this, we investigate multiple strategies for training a dual-encoder model starting from a language model pretrained on a large text corpus. Compared to public dual-encoder models such as CLIP and OpenCLIP, the model trained with our best adaptation strategy achieves a significantly higher ranking similarity for paraphrased queries while maintaining similar zero-shot classification and retrieval accuracy.

==> sections/tables/dataset_samples_old.tex <==
\begin{figure}[!t]
\centering
% \small
\footnotesize
\begin{tabular}{|m{1.8cm}|c|c|}
\toprule
\centering{Image} & Caption & Score
\tabularnewline
\midrule
{\includegraphics[width=\cellwidthb cm, height=\cellwidthb cm]{samples/000000055150.jpg}} &
\makecell[l]{original : \textit{Two children smiling on top} \\  \textit{of luggage in parking lot}. \\ paraphrase: \textit{Two kids grinning atop} \\  \textit{suitcases in a parking lot.}} & 5
\tabularnewline
\midrule
{\includegraphics[width=\cellwidthb cm, height=\cellwidthb cm]{samples/000000206027.jpg}} &
\makecell[l]{original : \textit{A slice of pizza  that is on} \\ \textit{top of a napkin.} \\ paraphrase: \textit{A piece of  pizza that is} \\  \textit{on top of a paper towel.}} & 4
\tabularnewline
\midrule
{\includegraphics[width=\cellwidthb cm, height=\cellwidthb cm]{samples/000000364297.jpg}} &
\makecell[l]{original: \textit{There is a cat laying down} \\  \textit{on a keyboard.}  \\ paraphrase: \textit{A cat is stretched out on} \\ \textit{a keyboard.} } & 3
\tabularnewline
\midrule
{\includegraphics[width=\cellwidthb cm, height=\cellwidthb cm]{samples/000000515577.jpg}} &
\makecell[l]{original : \textit{Two skiers prepare to make} \\  \textit{their  way past an embankment.} \\ paraphrase: \textit{Two skiiers are getting} \\ \textit{ready to  go around a big hill.}} & 2
\tabularnewline
\midrule
{\includegraphics[width=\cellwidthb cm, height=\cellwidthb cm]{samples/000000003553.jpg}} &
\makecell[l]{original : \textit{A person skating on some} \\  \textit{pieces of wood.} \\ paraphrase: \textit{A person skating on  a} \\  \textit{rink made of ice.}} & 1
\tabularnewline
\bottomrule
\end{tabular}
\vspace{0.1cm}
\caption{\textbf{Paraphrased Text-Image Retrieval dataset samples.} We show five sample images (left), their original captions and the corresponding paraphrases generated by GPT-3 (middle), and the human-provided semantic similarity scores (right). A semantic similarity score of 5 indicates that the paraphrase has an identical meaning to the original caption.}
    \label{fig:para_samples}
\end{figure}

==> sections/tables/laion_400m_results_detailed.tex <==
\begin{table*}[t]
\begin{tabular}{*l ^c | ^c ^c ^c ^c ^c ^c | ^c ^c }
& &
\multicolumn{6}{c|}{\textbf{zero-shot transfer}} &
\multicolumn{2}{c}{\textbf{paraphrased retrieval}} \\
& &
\multicolumn{2}{c|}{\scriptsize classification} & 
\multicolumn{2}{c|}{\scriptsize image retrieval} &
\multicolumn{2}{c|}{\scriptsize text retrieval} &
% \scriptsize lin-probe & \multicolumn{1}{c|}{\scriptsize fine-tune} & 
% \multicolumn{2}{c|}{\scriptsize captioning} &
% \scriptsize vqa 
&  
\\
model & dataset & 
\scriptsize IN-1K & \multicolumn{1}{c|}{\scriptsize VTAB+} & 
\scriptsize Flickr30k & \multicolumn{1}{c|}{\scriptsize COCO} & 
\scriptsize Flickr30k & \multicolumn{1}{c|}{\scriptsize COCO} & 
\scriptsize COCO & \scriptsize COCO + 128K
\\
\shline
CLIP~\cite{radford2021learning} & WIT-400M &
\better{63.3} & 45.5 & 
58.8 & 30.4 &
77.6 & 50.1 &
58.1 & 42.6
\\
OpenCLIP \cite{cherti2022reproducible} & LAION-400M &
62.9 & 45.8 &
\better{61.7} & \better{35.3} &
\better{79.0} & \better{52.5} &
59.5 & 42.5 
\\
OpenCLIP* & LAION-400M  &
62.4 & \better{47.0} &
60.6 & 34.7 &
78.6 & 51.1 &
- & - 
\\
\hline
Ours (6-layers) & LAION-400M  &
60.5 & 46.6 &
59.9 & 33.9 &
77.1 & 49.1 &
- & -
 \\
Ours (9-layers) & LAION-400M  &
60.4 & 46.4 &
60.8 & 34.6 &
76.9 & 51.0 &
- & - 
 \\
\end{tabular}

\caption{\textbf{Adaptation at Scale.} We compare our method with baselines at scale for multiple zero-shot tasks: classification, retrieval (R@1), and paraphrased retrieval (JS@10) . All models use ViT-B/32 as visual backbone and are trained for 32 epochs on the specified dataset. OpenCLIP* denotes our reproduction of \cite{cherti2022reproducible}. For VTAB+, we report the average top-1 accuracy over 35 tasks following the setup in \cite{schuhmann2022laionb}.
}
\label{tab:scaling}
\end{table*}




\begin{table*}[t]
\begin{tabular}{*l ^c | ^c ^c ^c ^c ^c ^c | ^c ^c  ^c ^c}
& &
\multicolumn{6}{c|}{\textbf{zero-shot transfer}} &
\multicolumn{4}{c}{\textbf{paraphrased retrieval}} \\
& &
\multicolumn{2}{c|}{\scriptsize classification} & 
\multicolumn{2}{c|}{\scriptsize image retrieval} &
\multicolumn{2}{c|}{\scriptsize text retrieval} &
% \scriptsize lin-probe & \multicolumn{1}{c|}{\scriptsize fine-tune} & 
% \multicolumn{2}{c|}{\scriptsize captioning} &
% \scriptsize vqa 
\multicolumn{4}{c|}{\scriptsize paraphrased text-image retrieval}   
\\
model & dataset & 
\scriptsize IN-1K & \multicolumn{1}{c|}{\scriptsize VTAB+} & 
\scriptsize Flickr30k & \multicolumn{1}{c|}{\scriptsize COCO} & 
\scriptsize Flickr30k & \multicolumn{1}{c|}{\scriptsize COCO} & 
\multicolumn{2}{c|}{\scriptsize COCO} & \multicolumn{2}{c|}{\scriptsize COCO + 128K}
\\
~ & ~ & 
\multicolumn{2}{c|}{\scriptsize Top-1 Acc} &
\multicolumn{2}{c|}{\scriptsize R@5} & 
\multicolumn{2}{c|}{\scriptsize R@5} &
\scriptsize AO@10 & \scriptsize JS@10 &
\scriptsize AO@10 & \scriptsize JS@10
\\
\shline
CLIP\cite{radford2021learning} & WIT-400M &
\better{63.3} & 45.5 & 
83.4 & 56.0 &
94.6 & 74.9 &
67.0 & 58.1 &
52.8 & 42.6
\\
OpenCLIP \cite{cherti2022reproducible} & LAION-400M &
62.9 & 45.8 &
85.5 & 60.9 &
94.0 & 76.7 &
68.1 & 59.5 &
51.5 & 42.5 
\\
OpenCLIP* & LAION-400M  &
62.4 & \better{47.0} &
84.1 & 60.0 &
94.6 & 75.3 &
68.4 & 59.9  &
53.0 & 43.6  
\\
\hline
Ours (6-layers) & LAION-400M  &
60.5 & 46.6 &
84.0 & 60.0 &
93.8 & 74.8 &
73.7 & 66.1 &
60.2 & 50.8
 \\
Ours (9-layers) & LAION-400M  &
60.4 & 46.4 &
84.7 & 60.2 &
92.9 & 75.4 &
73.5 & 65.7  &
59.6 & 50.9
 \\
\end{tabular}

\caption{\textbf{Adaptation at Scale.} R@5
}
\label{tab:scaling}
\end{table*}

==> sections/tables/tables_detailed.tex <==
\begin{table*}[!t]
\begin{center}
% \small 	
\footnotesize
% \scriptsize
\vspace{-0.cm}
\begin{tabular}{ccc|ccccccccc}
\toprule
~ & ~ &  ~ &  \multicolumn{1}{c}{Zero-shot}   &  \multicolumn{4}{c}{Text Retrieval}   &  \multicolumn{4}{c}{Image Retrieval} 
\tabularnewline
\midrule
  \multirow{2}{*}{Img}   & \multirow{2}{*}{Img Init} &  \multirow{2}{*}{Text} & \multicolumn{1}{c}{ImageNet} & \multicolumn{2}{c}{Flickr30k} & \multicolumn{2}{c}{COCO val}  & \multicolumn{2}{c}{Flickr30k} & \multicolumn{2}{c}{COCO val} 
\tabularnewline
~ & ~ & ~ &   {Acc}   & R@1 & R@5   & R@1 & R@5  & R@1 & R@5 & R@1 & R@5 
\tabularnewline
\midrule
 \multirow{10}{*}{{RN50}}  & \multirow{4}{*}{{Random}} &  Baseline & 33.6 & 47.5 & 75.8 & 19.4 & 42.0 & 43.0 & 71.8 & 18.9 & 41.5
\tabularnewline
~ & ~ & Locked & \ccb 20.1  & \ccb 31.1  & \ccb  60.9  & \ccb 12.4  & \ccb 31.8 & \ccb 28.1  & \ccb  55.4  & \ccb 11.9  & \ccb  27.6  \tabularnewline
~ & ~ & Finetune & \ccb 33.2 & \ccb 50.1 & \ccb 76.3 & \ccb 20.8 & \ccb  44.8 & \ccb 44.2 & \ccb 73.0 & \ccb 19.4 & \ccb 34.2 %% 
\tabularnewline
~ & ~ & Bottleneck Adapter & 21.9 & 32.7 & 62.4 & 13.0 & 32.2 & 29.6 & 58.1 &  12.3 & 29.5
\tabularnewline
~ & ~ & Alignment Layers & \ccb 33.7 & \ccb 54.7 & \ccb  80.5 & \ccb 23.9 & \ccb 47.7 & \ccb 49.7  & \ccb 76.5  & \ccb 20.5 & \ccb 44.5 
\tabularnewline
\cmidrule{2-12}
 ~  & \multirow{5}{*}{{ImageNet}} & Baseline &  36.9  & 48.5 & 78.3  & 22.5 & 46.3  & 48.2 & 73.1 & 22.4 & 45.8 
\tabularnewline
~ & ~ & Locked & \ccb  30.6 & \ccb 44.8  & \ccb 73.2   & \ccb  21.9 & \ccb 46.2 & \ccb 40.8  & \ccb 67.7   & \ccb 20.3  & \ccb  43.3  \tabularnewline
~ & ~ & Finetune & \ccb 37.3 & \ccb 51.6 & \ccb 79.5  & \ccb 24.2 & \ccb 47.3 & \ccb 48.8 & \ccb 75.7  & \ccb 22.7 & \ccb 46.2 
\tabularnewline
~ & ~ & Bottleneck Adapter & 33.2 & 52.1 & 78.6 & 25.0 & 49.4 & 46.8 & 75.0 &  22.4 & 46.8 
\tabularnewline
~ & ~ & Alignment Layers &  \ccb 37.8  & \ccb 54.5 & \ccb 81.1 & \ccb 26.7  & \ccb 51.3 & \ccb 50.6 & \ccb 76.9 & \ccb  24.0 & \ccb 48.0 
\tabularnewline
\midrule
 \multirow{10}{*}{{ViT-B/32}}  & \multirow{4}{*}{{Random}} &  Baseline & 29.0 & 43.2 & 68.1 & 16.6 & 37.5 & 41.0 & 67.2 &  16.0 & 35.8   
\tabularnewline
~ & ~ & Locked & \ccb 18.7  & \ccb 27.3  & \ccb 57.6 & \ccb 11.7  & \ccb  29.4  & \ccb 26.1  & \ccb 52.9   & \ccb 10.2  & \ccb  25.8 \tabularnewline
~ & ~ & Finetune & \ccb 28.5 & \ccb 44.4 & \ccb 70.2 & \ccb 17.8 & \ccb 38.1  & \ccb 40.9  & \ccb 67.7 & \ccb 15.5 & \ccb 34.9 
\tabularnewline
~ & ~ & Bottleneck Adapter & 18.8 & 30.2 &  57.8 & 11.4 &  28.7 & 26.2 & 53.3  &  9.2 & 25.5 
\tabularnewline
~ & ~ & Alignment Layers & \ccb 29.0 & \ccb 45.6  & \ccb 72.2 & \ccb 18.2 & \ccb 40.1  & \ccb 41.2  & \ccb 69.7 & \ccb 15.9 & \ccb 35.8 
\tabularnewline
% \cline{2-8}
\cmidrule{2-12}
 ~  & \multirow{4}{*}{{ImageNet}} & Baseline & 36.8 & 52.3 & 77.8 & 20.8 & 45.5 & 49.7 & 75.1 & 20.0 & 42.0 
\tabularnewline
~ & ~ & Locked & \ccb 30.2  & \ccb 42.9  & \ccb  71.6  & \ccb  16.5 & \ccb 38.6 & \ccb 39.2  & \ccb  66.9  & \ccb  16.0 & \ccb  38.6  \tabularnewline
~ & ~ & Finetune & \ccb 36.3 & \ccb 53.2 & \ccb 78.1 & \ccb 21.0 & \ccb 45.1  & \ccb 49.9 & \ccb 77.3 & \ccb 19.8 & \ccb 40.8 %%
\tabularnewline
~ & ~ & Bottleneck Adapter & 30.7 & 42.3 & 70.9 & 17.2  &  38.8 & 39.2 & 67.3 & 15.1  &  36.3 
\tabularnewline
~ & ~ & Alignment Layers & \ccb 37.5 & \ccb 54.6  & \ccb 80.7  & \ccb 21.8 & \ccb 46.4 & \ccb 51.9  & \ccb 80.0  & \ccb 20.6  
 & \ccb 45.9
\tabularnewline
\bottomrule
\end{tabular}
\end{center}
\caption{Accuracy and stability performance of different models trained on CC12M.}\label{tb:cc12m_acc}
\end{table*}

\begin{table}[!t]
\begin{center}
\setlength{\tabcolsep}{1.4pt} % Default value: 6pt
% \small 	
\footnotesize
% \scriptsize
\vspace{-0.cm}
\begin{tabular}{ccc|cccc}
\toprule
~ & ~ &  ~ &  \multicolumn{4}{c}{Para Rank Sim}
\tabularnewline
\midrule
  \multirow{2}{*}{Img}   & \multirow{2}{*}{Img Init} & \multirow{2}{*}{Text} & \multicolumn{2}{c}{COCO} & \multicolumn{2}{c}{COCO + 128K}
\tabularnewline
~ & ~ & ~ &  AO@10  & JS@10 &  AO@10  & JS@10
\tabularnewline
\midrule
 \multirow{10}{*}{{RN50}}  & \multirow{5}{*}{{Random}} &  Baseline & 51.7  & 43.4 & 34.6  & 27.2
\tabularnewline
~ & ~ & Locked &  \ccb 68.6  & \ccb  60.6  & \ccb  54.2 & \ccb  45.4 \tabularnewline
~ & ~ & Finetune & \ccb 53.0 & \ccb 44.9 & \ccb 35.1 & \ccb 28.1  %% 
\tabularnewline
~ & ~ & Adapter &  67.4 & 60.3  &  53.9 &  43.9 %%
\tabularnewline
~ & ~ & Align Layer &  \ccb 69.0 & \ccb 60.9 & \ccb 55.3 & \ccb 46.3
\tabularnewline
\cmidrule{2-7}
 ~  & \multirow{5}{*}{{ImageNet}} & Baseline &  53.7 &  44.9 & 35.7 & 28.1 
\tabularnewline
~ & ~ & Locked & \ccb 69.2  & \ccb 61.4  & \ccb  55.5  & \ccb  46.1 \tabularnewline
~ & ~ & Finetune & \ccb 55.3 & \ccb  45.1 & \ccb 36.4 & \ccb 28.3 %%
\tabularnewline
~ & ~ & Adapter  & 68.6 &  60.7  & 54.5 & 45.3 
\tabularnewline
~ & ~ & Align Layer & \ccb 69.8 & \ccb 61.2 & \ccb 55.3 & \ccb 46.0
\tabularnewline
\midrule
 \multirow{10}{*}{{ViT-B/32}}  & \multirow{5 }{*}{{Random}} &  Baseline  & 50.9  &  42.5  & 33.8 & 26.4
\tabularnewline
~ & ~ & Locked & \ccb 65.6 & \ccb  56.9  & \ccb  52.0 & \ccb  42.9 \tabularnewline
~ & ~ & Finetune & \ccb 51.9 & \ccb 44.9 & \ccb 34.0 & \ccb 26.7 %%
\tabularnewline
~ & ~ & Adapter & 65.5 &  57.0 & 52.7 & 43.1 
\tabularnewline
~ & ~ & Align Layer & \ccb 68.3 & \ccb 60.2 & \ccb 55.2 & \ccb 46.1 
\tabularnewline
% \cline{2-8}
\cmidrule{2-7}
 ~  & \multirow{5}{*}{{ImageNet}} & Baseline & 53.2  & 44.6 & 35.5 & 28.0  
\tabularnewline
~ & ~ & Locked & \ccb  66.6 & \ccb 58.6   & \ccb  53.4 & \ccb  43.9 \tabularnewline
~ & ~ & Finetune & \ccb 53.9  & \ccb 44.5  & \ccb 35.6 & \ccb 28.4 %%
\tabularnewline
~ & ~ & Adapter & 66.8 & 58.1  & 52.8 & 43.4  
\tabularnewline
~ & ~ & Align Layer & \ccb 68.8 & \ccb 60.7 & \ccb 55.1 & \ccb 45.9
\tabularnewline
\bottomrule
\end{tabular}
\end{center}
\caption{}\label{tb:cc12m_para_rank_sim}
\end{table}

\begin{table}[!t]
\begin{center}
\setlength{\tabcolsep}{1.4pt} % Default value: 6pt
% \small 	
\footnotesize
% \scriptsize
\vspace{-0.cm}
\begin{tabular}{ccc|cc}
\toprule
~ & ~ &  ~ &  \multicolumn{2}{c}{Semantic Text Similarity}
\tabularnewline
\midrule
  \multirow{2}{*}{Img}   & \multirow{2}{*}{Img Init} & \multirow{2}{*}{Text} & \multicolumn{2}{c}{STS-B} 
\tabularnewline
~ & ~ & ~ &  Pearson/\%  & Spearman/\% \tabularnewline
\midrule
 \multirow{10}{*}{{RN50}}  & \multirow{5}{*}{{Random}} &  Baseline & 68.3  & 68.2 \tabularnewline
~ & ~ & Locked &  \ccb 82.8  & \ccb  83.9    \tabularnewline
~ & ~ & Finetune & \ccb 71.0 & \ccb 69.9  %% 
\tabularnewline
~ & ~ & Adapter & 73.6  &  75.0    %%
\tabularnewline
~ & ~ & Align Layer &  \ccb 76.7  & \ccb 78.8
\tabularnewline
\cmidrule{2-5}
 ~  & \multirow{5}{*}{{ImageNet}} & Baseline & 68.4  & 68.5 \tabularnewline
~ & ~ & Locked & \ccb 81.6  & \ccb 83.1  \tabularnewline
~ & ~ & Finetune & \ccb 69.2 & \ccb 75.0 \tabularnewline
~ & ~ & Adapter  & 73.6 &  75.8 \tabularnewline
~ & ~ & Align Layer & \ccb 76.7 & \ccb 78.7
\tabularnewline
\midrule
 \multirow{10}{*}{{ViT-B/32}}  & \multirow{5}{*}{{Random}} &  Baseline  & 71.8  & 71.6 \tabularnewline
~ & ~ & Locked & \ccb  82.1 & \ccb 83.3     \tabularnewline
~ & ~ & Finetune & \ccb 72.4  & \ccb 72.9    \tabularnewline
~ & ~ & Adapter & 82.2 &  83.4 \tabularnewline
~ & ~ & Align Layer & \ccb 79.0 & \ccb 79.6 \tabularnewline
% \cline{2-8}
\cmidrule{2-5}
 ~  & \multirow{5}{*}{{ImageNet}} & Baseline &  70.0 & 69.7 \tabularnewline
 ~ & ~ & Locked & \ccb 81.1 & \ccb 82.9  \tabularnewline
~ & ~ & Finetune & \ccb 72.1 & \ccb 72.9  %%
\tabularnewline
~ & ~ & Adapter & 81.7 &  83.2
\tabularnewline
~ & ~ & Align Layer & \ccb 78.9 & \ccb 80.0 \tabularnewline

\bottomrule
\end{tabular}
\end{center}
\caption{}\label{tb:cc12m_stsb}
\end{table}

\begin{table}[!t]
\begin{center}
\small 	
% \scriptsize
% \footnotesize
\vspace{-0.cm}
\begin{tabular}{ccccccc}
\toprule
 ~  & ~ &  \multicolumn{5}{c}{$L_2$} \tabularnewline
   \cmidrule{3-7}
 Img Init & ~ &  0 & 2 & 4 & 6 &  8  \tabularnewline
  \midrule
 \multirow{2}{*}{Random} & R@5 &  25.8 & 33.1 & 35.4 & 35.8 &  36.4  \tabularnewline
  ~ & AO@10 &  52.0 & 55.4 & 55.5 & 55.2 &  55.3  \tabularnewline
 \midrule
  \multirow{2}{*}{ImageNet} & R@5 &  36.0 & 41.6 & 42.9 & 44.4 & 44.2   \tabularnewline
  ~ & AO@10 &  53.4 & 55.1 & 54.9 & 55.4 & 54.6  \tabularnewline
 \bottomrule
\end{tabular}
\end{center}
\caption{Retrieval accuracy and paraphrase ranking similarity versus the number of alignment layers $L_2$ on COCO Caption. All models are trained with ViT-B/32 image tower on CC12M.}
\label{tb:cc12m_L2}
% \vspace{-0.2cm}
\end{table}
